Weighted Reservoir Sampling With Replacement from Data Streams

In this work, we present a new random sampling method for data streams where the probability of an element's inclusion in the sample is proportional to a weight associated with that element. Our method is based on sampling with replacement, although most of the literature on this topic has focused on sampling without replacement. Our algorithm generates a weighted random sample in one pass over a population of unknown size. At any point in time, the sample is representative of the population seen so far and can be directly used by other modules without requiring any post-processing. We formally prove the correctness and efficiency of our method. An experimental analysis shows the performance of our method in practice when compared to state-of-the-art methods.

==> sections/our_contribution_v1.tex <==
\section{Our Method}
\label{sec:our_method}
\begin{enumerate}
	\item proof for the correctness of our method.
	\item proof for the cost of add of our method.
	\item Highlight the optimality for get.
	\item Highlight the optimality for merge.
	      
\end{enumerate}


\mynote[to=Faz]{Add here the description of the variables used in Algorithm~\ref{alg:our}
}
\begin{algorithm}[h!]
	\caption{\our}
	\label{alg:our}
	\KwInput{$\mathcal{S}$, $N$, $m$.}
	$(e_1,w_1) \gets \mathcal{S}_1$\;
	$\mathcal{R} \gets [\underbrace{e_1, e_1, \dots, e_1}_{m \text{ times}}]$; $W \gets w_1$; $W_{\text{skip}} \gets w_1$\;
	\For{$t = 2$ \KwTo $N$}{
		$(e_t, w_t) \gets \mathcal{S}_t$\;
		$W \gets W + w_t$\;
		\If{$W \geq W_{\text{skip}}$}{
			$q \sim U(0,1)$\;
			$W_{\text{skip}} \gets \frac{W}{q^{\frac{1}{m}}}$\;
			$k \sim B_{>0}\left(m,\frac{w_t}{W}\right)$\;
			Insert $e_t$ in $k$ distinct indices in $\mathcal{R}$ chosen uniformly at random\;
		}
	}
	\Return $\left(\mathcal{R}, W\right)$\;
\end{algorithm}
Algorithm~\ref{alg:our} provides the pseudocode for our \our method. 
The algorithm processes the first $N$ items of an input stream $S$ while maintaining a reservoir $\mathcal{R}$ of fixed size $m$ in each iteration.

The algorithm begins by initializing the reservoir $\mathcal{R}$ to contain $m$ copies of the first stream element $e_1$ (line 2). 
The total cumulative weight $W$ and the initial skip threshold $W_{skip}$ are both set to the weight of this first item, $w_1$ (line 2).

The algorithm then iterates through the remaining items of the stream from $t=2$ to $N$ (line 3). 
In each iteration, the current item $(e_t, w_t)$ is retrieved, and its weight $w_t$ is added to the cumulative total weight $W$ (lines 4--5).

The core of the algorithm's efficiency lies in its skipping mechanism. 
The algorithm only considers processing an item if the total weight $W$ has reached or surpassed the $W_{skip}$ threshold (line 6). 

\mynote[from=Faz,to=Adri]{Cite the paper that presented the skipping technique the first time.}
\faz{This check efficiently simulates the cumulative probability of rejecting a sequence of items without processing each one individually.}

If the condition in line 6 is met, the algorithm ``\textit{accepts}'' the current item $e_t$ and proceeds to update the reservoir.
First, it determines the \emph{next} skip threshold by drawing a uniform random number $q \sim U(0, 1)$ and setting $W_{skip} \gets W / q^{1/m}$ (lines 7--8). 
This new threshold defines the minimum total weight that must be accumulated before the \emph{next} item can be processed.

Next, the number of copies $k$ for $e_t$ to be inserted into the reservoir is drawn from $B_{>0}(m, \frac{w_t}{W})$, a Binomial distribution truncated at zero (line 9). 
The truncation guarantees that the element $e_t$ is selected to replace at least one element ($k>0$) in the reservoir $\mathcal{R}$.

Finally, the element $e_t$ is inserted into $k$ distinct positions in $\mathcal{R}$, chosen uniformly at random, replacing the elements previously at those positions (line 10). The algorithm then continues to the next item in the stream, or returns the final reservoir $\mathcal{R}$ and total weight $W$ if exactly $N$ stream items have been read (line 11).

We now prove the correctness of the \textit{add} operation of the WRSWR-SKIP algorithm.

\begin{lemma}
	%WRSWR-SKIP maintains an unbiased weighted random sample with replacement throughout the sampling process.
    Algorithm~\ref{alg:our} 
	
	\begin{proof}
		Let $W_n$ denote the total accumulated weight of the stream after processing $n$ elements. In the standard weighted reservoir sampling with replacement, a new element $e_i$ with weight $w_i$ is selected to replace items in the reservoir based on a draw from a Binomial distribution $\text{Bin}(m, w_i/W_i)$. Consequently, the probability that an element $e_i$ is \textit{not} selected (i.e., 0 copies are inserted) is:
		\[
			P(\text{Reject } e_i) = \left(1 - \frac{w_i}{W_i}\right)^m = \left(\frac{W_i - w_i}{W_i}\right)^m = \left(\frac{W_{i-1}}{W_i}\right)^m
		\]
		The probability of consecutively rejecting the next $t$ elements $e_{n+1}, \dots, e_{n+t}$ is
		\begin{align*}
			P(\text{Skip} \ge t) & = \prod_{j=1}^{t} P(\text{Reject } e_{n+j}) = \prod_{j=1}^{t} \left(\frac{W_{n+j-1}}{W_{n+j}}\right)^m = \left( \frac{W_n}{W_{n+t}} \right)^m 
		\end{align*}
		To simulate the binomial sampling, we can generate a random variable $q \sim U(0, 1)$ and continue skipping elements as long as the cumulative probability remains higher than $q$:
		\[
			\left( \frac{W_n}{W_{n+t}} \right)^m > q \implies W_{n+t} < \frac{W_n}{q^{1/m}}
		\]
		The algorithm implements this by computing the threshold $T = W_n / q^{1/m}$ and accumulating weights until $W_{n+t} \ge T$. 
		
		When this condition is met, the element $e_{n+t}$ is the first in the sequence to be selected. The logic conditions on the event that the number of inserted copies $k$ is non-zero (otherwise the skip would have continued), therefore, $k$ must be drawn from a truncated Binomial distribution at $k = 0$. Thus, the algorithm ensures that the sampling process remains unbiased.
	\end{proof}
\end{lemma}

One particularly useful measure to evaluate the efficiency of a reservoir sampling algorithm is the expected number of random generations needed.

\begin{lemma}
	
	%The expected number of random operations produced by WRSWR-SKIP after observing $N$ elements of the stream is $O\left(m \log\frac{W_N}{W_0} \right)$.
    Algorithm~\ref{alg:our} requires $O\left(m \log\frac{W}{w_1} \right)$ random number generations in expectation.
	\begin{proof}
        Let's define $X$ as the random variable representing the number of random number generations performed by Algorithm~\ref{alg:our} at the $N$-th iteration.
	    %Take $X$ as the r.v. of random operations computed by the algorithm, then
    	\begin{align*} 
    		\mathbb{E}(X) & = \sum_{t=1}^N \left(1-\left(\frac{W_{t-1}}{W_{t}}\right)^m\right)  \left(2 + \mathbb{E}\left(\text{Bin}\left(m, \frac{W_{t} - W_{t-1}}{W_{t}}\right)\right)\right) \\
    		              & = \sum_{t=1}^N \left(1-\left(\frac{W_{t-1}}{W_{t}}\right)^m\right)\left(2 + m\frac{W_{t} - W_{t-1}}{W_{t}} \right).
    	\end{align*} 
    	Since $\left(1-\left(\frac{W_{t-1}}{W_{t}}\right)^m\right)$ is the probability to accept at least once the $t$-th element of the stream and, when this happens, the skip is recomputed, a binomial experiment is performed and $\mathbb{E}\left(\text{Bin}\left(m, \frac{W_{t} - W_{t-1}}{W_{t}}\right)\right)$ elements are substituted on average in the reservoir.
    	Notice that 
    	\begin{align*} 
    		\mathbb{E}\left(X\right) \leq  3 m \sum_{t=1}^N \left(\frac{W_{t} - W_{t-1}}{W_{t}}\right) < 3m\sum_{t=1}^N \log \frac{W_{t}}{W_{t-1}} = 3m\log \frac{W_{N}}{W_0}.
    	\end{align*} 
    	The first inequality follows from the fact that if we let \(x = \tfrac{W_{t-1}}{W_{t}} \in \mathbb{R}_{(0,1)}\), the factor \((1 - x^m)(2 + m(1 - x))\) is maximized by \(3m(1 - x)\), and the second from the convexity of the $\log$ function. Therefore, $\mathbb{E}\left(X\right) = O\left(m \log \frac{W_N}{W_0}\right)$ as stated.
	\end{proof}
\end{lemma}

As described in Algorithm~\ref{alg:our}, \our outputs both a reservoir $\mathcal{R}$ and the total weight of the input stream $W$.
A key property of this reservoir $\mathcal{R}$ is that it is an actual unbiased sample of the stream, making it immediately usable for further analysis.
In contrast, the structure used by \textbf{WRAEXP-J}~\cite{shekelyan2023EDBT} is not an unbiased sample itself and requires post-processing to extract one.
Moreover, the positions of the elements within our reservoir are uniformly random. These exactly two properties are also possessed by the reservoir used by the \textbf{WRSWR} baseline.
%Unbiased sample with repetitions.

\begin{algorithm}[h!]
	\caption{Merging Reservoirs from \our}
	\label{alg:our_merge}
	\KwInput{$\left(\mathcal{R}_1, W_1\right), \left(\mathcal{R}_2, W_2\right), \cdots, \left(\mathcal{R}_n, W_n\right)$.}
	$W \gets \sum_{i \in [n]} W_i$\;
    $m \gets \min_{i \in [n]}{|\mathcal{R}_i}|$\;
    $\left[k_1, k_2, \cdots, k_n \right] \sim \text{Mult}\left(m, \left[\frac{W_1}{W}, \frac{W_2}{W}, \cdots, \frac{W_n}{W}\right]\right)$\;
    $\mathcal{R} \gets \bigoplus_{i \in [n]} \mathcal{R}_i[1:k_i]$\;
    \Return $\left(\mathcal{R}, W\right)$\;
\end{algorithm}
\mynote[to=Faz]{Describe line by line Algorithm~\ref{alg:our_merge}
}

\begin{lemma}
Merging $k$ reservoirs of size $m_1, \dots, m_k$ into one of size $\min{(m_1, \dots, m_k)}$ requires $O(k)$ random operations.
    \begin{proof}
        Suppose to track the total weight of each of the streams $W_1, \dots, W_k$.
    \end{proof}
\end{lemma}


% % FIRST TABLE 
% \begin{table}[h!]
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% operation & WRSWR & WRSWR-BIN & WRAEXP-J & WRSWR-SKIP \\ \hline
% add & $O(Nm)$ & $O(N+m\log\frac{W_N}{W_0})$ & ? & $O(m\log\frac{W_N}{W_0})$ \\ \hline
% get & $O(1)$ & $O(1)$ & $O(m)$ & $O(1)$ \\ \hline
% merge & $O(k)$ & $O(k+m)$ & $O(k+m)$ & $O(k)$ \\ \hline
% \end{tabular}
% \end{table}


\begin{table}[htbp]
\centering
\small % <-- Still recommend using \small
% Force table to \columnwidth and let LaTeX figure out the spacing
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}} l cccc} 
\toprule
\textbf{Op.} & \textbf{WRSWR} & \textbf{WRSWR-BIN} & \textbf{WRAEXP-J} & \textbf{WRSWR-SKIP} \\
\midrule
add & $O\left(Nm\right)$ & $O\left(N+m\log\frac{W_N}{W_1}\right)$ & $O\left(m\log \frac{N}{m}\right)^*$ & $O\left(m\log\frac{W_N}{W_1}\right)$ \\
get & $O\left(1\right)$ & $O\left(1\right)$ & $O\left(m\right)$ & $O\left(1\right)$ \\
merge & $O\left(n\right)$ & $O\left(n+m\right)$ & $O\left(n+m\right)$ & $O\left(n\right)$ \\
\bottomrule
\end{tabular*}
\caption{Time complexity of operations for each algorithm. $^*$According to ~\cite{efraimidis2006information} the complexity for WRAEXP-J holds under the i.i.d. assumption for the weight distribution.}
\label{tab:time_complexity_comparison}
\end{table}

\mynote[from=Faz]{I am going to explain the last colums of Table~\ref{tab:time_complexity_comparison}.}

==> sections/scheme.tex <==
\section{ScHeMe}
\label{sec:scheme}
\begin{enumerate}
    \item proof for the correctness of our method.
    \item proof for the cost of add of our method.
\end{enumerate}

